By the user, for the user: A user-centric approach to quantifying the privacy of websites

Third-party tracking is common on almost all commercially operated websites. Prior work has studied in detail the extent of third-party tracking on the web, detection of third-party trackers, and defending against third-party tracking. Existing research and tools have also attempted to inform web users of trackers and the extent of their privacy violations. However, existing tools do not take into account users' perceptions of and understanding of the extent of trackers on the web. Taking these factors into account is important for the usability of such tools so that users can be aware and protect themselves to a reasonable and necessary extent that aligns with their overall comfort with trackers. In this paper, we elicit user perceptions and preferences about different trackers on various websites through an online survey of 43 users. We use this data to bootstrap a privacy scoring system. This scoring system weights the usage of trackers and the dispersion of user data within a page to third parties, with the type of website being visited. Our work presents a proof-of-concept methodology and tool to calculate a user-centric privacy score with preliminary bootstrap user data. We conclude with concrete future directions.

==> algorithm2.tex <==
% \begin{algorithm}
% siteCategory $\longleftarrow$ GetSiteCategory()

% % \tcc{Update stored aggTPTScore for this site}
% storedAggTPTScore $\longleftarrow$ average( GetSiteAggTPTScore(), StoredAggTPTScore())\

% % \tcc{Get categorical privacy score}
% categoricalPrivScore $\longleftarrow$ GetCategoricalPercentile()\

% % \tcc{Get global privacy score}
% globalPrivScore $\longleftarrow$ GetGlobalPercentile()\

% % \tcc{Get privacy score}
% privacyScore $\longleftarrow$ average(categoricalPrivScore, globalPrivScore)\

% \caption{Calculating Privacy Score for a page}
% \end{algorithm}

==> conclusion.tex <==
\section{Conclusion}

In this project, we presented a tool that provides a comprehensive aggregation of the privacy metrics that matter the most to users. To achieve this, we conducted a user study whose results were used to build the scoring mechanism. The main findings of the user study were that in terms of awareness and attitude towards TPTs, was that not many users knew about session replay TPTs, but yet after finding out it became the TPT they felt the least comfortable with. On the other hand, most participants knew about advertising TPTs, as expected. Concerning the website categories, banking and adult websites are the types people think should not include too many TPTs. These were closely followed by healthcare websites.

The Google Chrome extension we built fully achieves its role as a privacy scoring mechanism for websites. It takes into account the study findings and seems to work well. The only limitation is the number of TPTs that are known to our database, which makes our extension catch less trackers compared to more established ad-blocking services.



==> future-work.tex <==
\section{Future work}
Manual capturing and labelling of TPTs and websites is a time-consuming process. However, it was necessary to label them to provide the information we need to run the system. In the future, this manual process could be automated.

The pilot study involved 43 participants, which is a relatively small pool of participants. In the future, conducting the study with more participants perhaps with people across continents would result in more generalized findings to further tune the system.

==> references.tex <==
@article{englehardt2015openwpm,
  title={OpenWPM: An automated platform for web privacy measurement},
  author={Englehardt, Steven and Eubank, Chris and Zimmerman, Peter and Reisman, Dillon and Narayanan, Arvind},
  journal={Manuscript, mar},
  year={2015}
}

@inproceedings{englehardt2015cookies,
  title={Cookies that give you away: The surveillance implications of web tracking},
  author={Englehardt, Steven and Reisman, Dillon and Eubank, Christian and Zimmerman, Peter and Mayer, Jonathan and Narayanan, Arvind and Felten, Edward W},
  booktitle={Proceedings of the 24th International Conference on World Wide Web},
  pages={289--299},
  year={2015},
  organization={International World Wide Web Conferences Steering Committee}
}

@inproceedings{guha2010challenges,
  title={Challenges in measuring online advertising systems},
  author={Guha, Saikat and Cheng, Bin and Francis, Paul},
  booktitle={Proceedings of the 10th ACM SIGCOMM conference on Internet measurement},
  pages={81--87},
  year={2010},
  organization={ACM}
}

@inproceedings{ihm2011towards,
  title={Towards understanding modern web traffic},
  author={Ihm, Sunghwan and Pai, Vivek S},
  booktitle={Proceedings of the 2011 ACM SIGCOMM conference on Internet measurement conference},
  pages={295--312},
  year={2011},
  organization={ACM}
}

@inproceedings{jackson2006protecting,
  title={Protecting browser state from web privacy attacks},
  author={Jackson, Collin and Bortz, Andrew and Boneh, Dan and Mitchell, John C},
  booktitle={Proceedings of the 15th international conference on World Wide Web},
  pages={737--744},
  year={2006},
  organization={ACM}
}

@inproceedings{jang2010empirical,
  title={An empirical study of privacy-violating information flows in JavaScript web applications},
  author={Jang, Dongseok and Jhala, Ranjit and Lerner, Sorin and Shacham, Hovav},
  booktitle={Proceedings of the 17th ACM conference on Computer and communications security},
  pages={270--283},
  year={2010},
  organization={ACM}
}

@inproceedings{jensen2007tracking,
  title={Tracking website data-collection and privacy practices with the iWatch web crawler},
  author={Jensen, Carlos and Sarkar, Chandan and Jensen, Christian and Potts, Colin},
  booktitle={Proceedings of the 3rd symposium on Usable privacy and security},
  pages={29--40},
  year={2007},
  organization={ACM}
}

@inproceedings{krishnamurthy2011privacy,
  title={Privacy leakage vs. protection measures: the growing disconnect},
  author={Krishnamurthy, Balachander and Naryshkin, Konstantin and Wills, Craig},
  booktitle={Proceedings of the Web},
  volume={2},
  number={2011},
  pages={1--10},
  year={2011}
}

@inproceedings{krishnamurthy2009leakage,
  title={On the leakage of personally identifiable information via online social networks},
  author={Krishnamurthy, Balachander and Wills, Craig E},
  booktitle={Proceedings of the 2nd ACM workshop on Online social networks},
  pages={7--12},
  year={2009},
  organization={ACM}
}

@inproceedings{krishnamurthy2009privacy,
  title={Privacy diffusion on the web: a longitudinal perspective},
  author={Krishnamurthy, Balachander and Wills, Craig},
  booktitle={Proceedings of the 18th international conference on World wide web},
  pages={541--550},
  year={2009},
  organization={ACM}
}

@inproceedings{krishnamurthy2006generating,
  title={Generating a privacy footprint on the internet},
  author={Krishnamurthy, Balachander and Wills, Craig E},
  booktitle={Proceedings of the 6th ACM SIGCOMM conference on Internet measurement},
  pages={65--70},
  year={2006},
  organization={ACM}
}

@inproceedings{roesner2012detecting,
  title={Detecting and defending against third-party tracking on the web},
  author={Roesner, Franziska and Kohno, Tadayoshi and Wetherall, David},
  booktitle={Proceedings of the 9th USENIX conference on Networked Systems Design and Implementation},
  pages={12--12},
  year={2012},
  organization={USENIX Association}
}

@inproceedings{eubank2013shining,
  title={Shining the floodlights on mobile web tracking-a privacy survey},
  author={Eubank, Christian and Melara, Marcela and Perez-Botero, Diego and Narayanan, Arvind},
  booktitle={Proceedings of the IEEE Workshop on Web},
  volume={2},
  year={2013}
}

@article{han2012study,
  title={A study of third-party tracking by mobile apps in the wild},
  author={Han, Seungyeop and Jung, Jaeyeon and Wetherall, David},
  journal={Univ. Washington, Tech. Rep. UW-CSE-12-03-01},
  year={2012}
}

@inproceedings{leon2013matters,
  title={What matters to users?: factors that affect users' willingness to share information with online advertisers},
  author={Leon, Pedro Giovanni and Ur, Blase and Wang, Yang and Sleeper, Manya and Balebako, Rebecca and Shay, Richard and Bauer, Lujo and Christodorescu, Mihai and Cranor, Lorrie Faith},
  booktitle={Proceedings of the ninth symposium on usable privacy and security},
  pages={7},
  year={2013},
  organization={ACM}
}

@inproceedings{mcdonald2010americans,
  title={Americans' attitudes about internet behavioral advertising practices},
  author={McDonald, Aleecia M and Cranor, Lorrie Faith},
  booktitle={Proceedings of the 9th annual ACM workshop on Privacy in the electronic society},
  pages={63--72},
  year={2010},
  organization={ACM}
}

@inproceedings{ur2012smart,
  title={Smart, useful, scary, creepy: perceptions of online behavioral advertising},
  author={Ur, Blase and Leon, Pedro Giovanni and Cranor, Lorrie Faith and Shay, Richard and Wang, Yang},
  booktitle={proceedings of the eighth symposium on usable privacy and security},
  pages={4},
  year={2012},
  organization={ACM}
}

@inproceedings{tan2018comparing,
  title={Comparing Hypothetical and Realistic Privacy Valuations},
  author={Tan, Joshua and Sharif, Mahmood and Bhagavatula, Sruti and Beckerle, Matthias and Mazurek, Michelle L and Bauer, Lujo},
  booktitle={Proceedings of the 2018 Workshop on Privacy in the Electronic Society},
  pages={168--182},
  year={2018},
  organization={ACM}
}

@article{binns2018measuring,
  title={Measuring Third-party Tracker Power across Web and Mobile},
  author={Binns, Reuben and Zhao, Jun and Kleek, Max Van and Shadbolt, Nigel},
  journal={ACM Transactions on Internet Technology (TOIT)},
  volume={18},
  number={4},
  pages={52},
  year={2018},
  publisher={ACM}
}

@inproceedings{hamed2013evaluation,
  title={Evaluation of third party tracking on the web},
  author={Hamed, Asma and Ayed, Hella Kaffel-Ben and Kaafar, Mohamed Ali and Kharraz, Ahmed},
  booktitle={8th International Conference for Internet Technology and Secured Transactions (ICITST-2013)},
  pages={471--477},
  year={2013},
  organization={IEEE}
}

@inproceedings{englehardt2016online,
  title={Online tracking: A 1-million-site measurement and analysis},
  author={Englehardt, Steven and Narayanan, Arvind},
  booktitle={Proceedings of the 2016 ACM SIGSAC conference on computer and communications security},
  pages={1388--1401},
  year={2016},
  organization={ACM}
}

@article{signanini2014ghostery,
  title={Ghostery},
  author={Signanini, JM and McDermott, B},
  year={2014}
}

@article{adblock, title={Adblock Plus: The world's No. 1 free ad blocker}, url={https://adblockplus.org/en/}, journal={Adblock Plus | The world's # 1 free ad blocker}, year={2019}}

@inproceedings{mayer2012third,
  title={Third-party web tracking: Policy and technology},
  author={Mayer, Jonathan R and Mitchell, John C},
  booktitle={2012 IEEE symposium on security and privacy},
  pages={413--427},
  year={2012},
  organization={IEEE}
}

@article{turk, url={https://www.mturk.com/}, title={Amazon Mechanical Turk}, journal={Amazon Mechanical Turk}, year={2019}}

@article{tracking-works, title={How does online tracking actually work?}, url={https://robertheaton.com/2017/11/20/how-does-online-tracking-actually-work/}, journal={Robert Heaton}, year={2017}}

@misc{alexa, title={The top 500 sites on the web The sites in the top sites lists are ordered by their 1 month Alexa traffic rank.The 1 month rank is calculated using a combination of average daily visitors and pageviews over the past month. The site with the highest combination of visitors and pageviews is ranked #1}, url={https://www.alexa.com/topsites}, journal={Alexa}, year={2018}}

@article{awis, title={AWIS | Alexa Web Information Service - Traffic Metrics for any Website}, 
  url={https://aws.amazon.com/awis/}, year={2019}
}

@article{sim-web-classification, title={SimilarWeb | Website Categorization API}, 
  url={https://www.similarweb.com/corp/developer/website_categorization_API}, year={2019}
}

@article{g-content, title={Google | Cloud Natural Language API: Content Categories}, 
  url={https://cloud.google.com/natural-language/docs/categories}, year={2019}
}


@article{tracking:pets2016,
  title =        {({Do} not) {Track} me sometimes: {Users'} contextual preferences for web tracking},
  author =       {William Melicher and Mahmood Sharif and Joshua Tan and Lujo Bauer and Mihai Christodorescu and Pedro Giovanni Leon},
  journal =      {Proceedings on Privacy Enhancing Technologies},
  year =         2016,
  issue =        2,
  month =        apr,
  copyright =    {authors},
  publisher =    {De Gruyter Open},
  doi =          {10.1515/popets-2016-0009},
  url =          {http://www.ece.cmu.edu/~lbauer/papers/2016/pets2016-online-tracking.pdf},
  keywords =     {privacy, human factors}
}

@inproceedings{bhagavatula2014leveraging,
  title={Leveraging machine learning to improve unwanted resource filtering},
  author={Bhagavatula, Sruti and Dunn, Christopher and Kanich, Chris and Gupta, Minaxi and Ziebart, Brian},
  booktitle={Proceedings of the 2014 Workshop on Artificial Intelligent and Security Workshop},
  pages={95--102},
  year={2014},
  organization={ACM}
}

@inproceedings{Orr:2012:AIJ:2381966.2381968,
 author = {Orr, Caitlin R. and Chauhan, Arun and Gupta, Minaxi and Frisz, Christopher J. and Dunn, Christopher W.},
 title = {An Approach for Identifying JavaScript-loaded Advertisements Through Static Program Analysis},
 booktitle = {Proceedings of the 2012 ACM Workshop on Privacy in the Electronic Society},
 series = {WPES '12},
 year = {2012},
 isbn = {978-1-4503-1663-7},
 location = {Raleigh, North Carolina, USA},
 pages = {1--12},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/2381966.2381968},
 doi = {10.1145/2381966.2381968},
 acmid = {2381968},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {advertisements, analytics, javascript, security},
} 

@inproceedings{lerner2016internet,
  title={Internet jones and the raiders of the lost trackers: An archaeological study of web tracking from 1996 to 2016},
  author={Lerner, Adam and Simpson, Anna Kornfeld and Kohno, Tadayoshi and Roesner, Franziska},
  booktitle={25th $\{$USENIX$\}$ Security Symposium ($\{$USENIX$\}$ Security 16)},
  year={2016}
}

@inproceedings{toubiana2010adnostic,
  title={Adnostic: Privacy preserving targeted advertising},
  author={Toubiana, Vincent and Narayanan, Arvind and Boneh, Dan and Nissenbaum, Helen and Barocas, Solon},
  booktitle={Proceedings Network and Distributed System Symposium},
  year={2010}
}

@inproceedings{fredrikson2010repriv,
  title={RePriv: Re-envisioning in-browser privacy},
  author={Fredrikson, Matthew and Livshits, Benjamin},
  booktitle={Proc. IEEE Symp. Security, Privacy (SP)(May 2011)},
  year={2010}
}

@inproceedings{guha2011privad,
  title={Privad: Practical privacy in online advertising},
  author={Guha, Saikat and Cheng, Bin and Francis, Paul},
  booktitle={USENIX conference on Networked systems design and implementation},
  pages={169--182},
  year={2011}
}

@inproceedings{dhawan2012priv3,
  title={Priv3: A third party cookie policy},
  author={Dhawan, Mohan and Kreibich, Christian and Weaver, Nicholas},
  booktitle={W3C Workshop: Do Not Track and Beyond},
  year={2012}
}

@inproceedings{kontaxis2012privacy,
  title={Privacy-preserving social plugins},
  author={Kontaxis, Georgios and Polychronakis, Michalis and Keromytis, Angelos D and Markatos, Evangelos P},
  booktitle={Presented as part of the 21st $\{$USENIX$\}$ Security Symposium ($\{$USENIX$\}$ Security 12)},
  pages={631--646},
  year={2012}
}

@article{roesner2012sharemenot,
  title={Sharemenot: Balancing privacy and functionality of third-party social widgets},
  author={Roesner, Franziska and Rovillos, Christopher and Kohno, Tadayoshi and Wetherall, David},
  journal={Usenix; login},
  year={2012}
}

@inproceedings{chanchary2015user,
  title={User perceptions of sharing, advertising, and tracking},
  author={Chanchary, Farah and Chiasson, Sonia},
  booktitle={Eleventh Symposium On Usable Privacy and Security ($\{$SOUPS$\}$ 2015)},
  pages={53--67},
  year={2015}
}
